Learning to Sample

Processing large point clouds is a challenging task. Therefore, the data is often sampled to a size that can be processed more easily. The question is how to sample the data? A popular sampling technique is Farthest Point Sampling (FPS). However, FPS is agnostic to a downstream application (classification, retrieval, etc.). The underlying assumption seems to be that minimizing the farthest point distance, as done by FPS, is a good proxy to other objective functions. We show that it is better to learn how to sample. To do that, we propose a deep network to simplify 3D point clouds. The network, termed S-NET, takes a point cloud and produces a smaller point cloud that is optimized for a particular task. The simplified point cloud is not guaranteed to be a subset of the original point cloud. Therefore, we match it to a subset of the original points in a post-processing step. We contrast our approach with FPS by experimenting on two standard data sets and show significantly better results for a variety of applications. Our code is publicly available at: https://github.com/orendv/learning_to_sample

==> Scenarios.tex <==
% \subsection{When and how to use \SNET}
%-------------------------------------              Extra large point clouds






























%MOVED BACK TO RESULTS_CLASSIFICATION

































% \noindent {\bfseries Extra large point clouds} \quad Assume you have a dataset of point clouds that are too large to train your network on, let us denote their size as XL. You used FPS to sub-sample the point clouds to a reasonable size, let's call that size $k$, and than you trained your network on those sub-sampled clouds. So now you have a network that learned to take a cloud of size $k$ and perform your task with some performance. How can you improve it? You could try to feed your network a XL point cloud, but that would not work since it was not trained for it (as we will soon demonstrate with PointNet as an example). So you take the fallowing steps, illustrated in Figure~ {\color{red}(Oren: don't have this figure yet)}: 1.You use the FPS-sampled $k$-sized point clouds to train \SNET, using your already-trained network as the task network. 2.You use \SNET to sample the XL point clouds to size $k$. 3. You train your network again, this time on the point clouds produced by \SNET.
% The newer version of your network, trained on \SNET's points, will produce better performance for your task.

% How do we know that? We tried it, on a small-scale simulation, as follows: We used FPS to sample ModelNet40 to $k=32$ points per point clouds, and trained PointNet vanilla {\color{red} (Oren: Should re-do it with PointNet, not vanila, since in the table we show the corresponding number for PointNet)} on those sampled points, this is our baseline. The accuracy of the baseline on the test set is 80.2\%. When we tried to feed this PointNet with points clouds of size $XL=1024$, the accuracy was just {\color{red}(Oren: Don't have this number yet but I remember it was not better)}. So we followed the receipt laid out above: 
% 1. We Trained \SNET, using the $32$-sized point clouds training set, and the baseline PointNet as the task network.
% 2. We sampled ModleNet40 again to size $k=32$, this time using \SNET.
% 3. We trained PointNet on the points sampled by \SNET.
% And, the accuracy on the test set improved to 84.7\%. There is no current way to achieve this accuracy which such a limited training capacity (training on point clouds of only $k=32$ points) without using \SNET.




%-------------------------------------            Limited inference resources}
\medskip
% \noindent {\bfseries Limited inference resources} \quad Assume your network's inference is too heavy, even though you have already simplified it as much as you could. If it's a PointNet-like network, its time complexity is dominated by its per-point convolution layers, and so is heavily dependent on the size of the input point cloud. Therefore, you need your network to work on point clouds of smaller size. You have 2 options: 1.Feed smaller point clouds to your existing network. 2.Re-train your network to work on smaller point clouds. You would want to use option 2 if you are certain about a specific input size you will always want to use, and if re-training your network is feasible, and option 1 otherwise.

% In both cases you will get better results by using \SNET as your sampling method: We already saw in Figure~\ref{fig:SampleNet_results} how the accuracy on a given PointNet is higher when feeding it \SNET's points than when feeding it FPS points. Table ~\ref{table:ReTrain} show us how the accuracy of PointNet is also higher when {\em training} it to work on the points sampled by \SNET, as oppose to FPS or randomly sampled points. Each of the numbers in this table represents a different PointNet, each trained and tested on point clouds of a specific size that was sampled with a specific sampling method. We can see for example, a PointNet that was both trained and tested on point clouds of just 16 points, achieved 85.6\% accuracy, when \SNET was used to sample the point clouds from 1024 points to 16 points, compared to only 76.7\% when FPS was used to sample the point clouds for training and testing.

% On point clouds of the same size, \SNET's has 12 times faster inference than PointNet. When cascading \SNET with a following PointNet, PointNet needs to process a lot less points, and therefore its inference is much faster. Table~\ref{table:params} demonstrates how we save most of the inference time by using \SNET. When fed the full 1024-large points clouds, PointNet performs 440 million floating point multiplications, but when feeding PointNet with only 16 points, this number drops to 7 million. \SNET that sample from 1024 to 16 points performs only 35 million floating point multiplications. Cascading them together, amount to 42 million FLOPs, which is 90\% reduction in inference time.





% {\color{red}(Oren: It  is not compared to FPS, it is compared to using PointNet on the full (1024-points) point clouds.}

% {\color{red}(Shai: We are 12 faster than PointNet-1024 but we could run FPS followed by PointNet-16 and then we'll be as fast but with accuracy 76\%. Correct? Need to be careful. Hmmmmm
% Okay, then the table should show 2 options. \SNET with PointNet16 and FPS with Point-16. Maybe show a couple of such pairs - that's the correct comparison. Maybe show these as points in a graph where the x-axis is the accuracy and y-axis is #Flops.

% I think we'll lose in this compariosn with re-training of PointNet for lower inputs, and win when PointNet is fixed (was trained on full inputs and fed with smaller). Because you can do FPS to 64 + PointNet instead of \SNET to 16 + PointNet. 

% Even with a fixed PointNet it doesn't make sense. Because why would you want to do any of those calculations on the client? just send the full Point cloud. No, that's too expensive. In terms of network bandwidth? If you don't have network problems, you will do the sampling on the cloud.

% But you always have bandwidth problems. Why transmit 1024 points if you can send only 16? I'm bothered by the first point you made. Running FPS-64+PointNet. So the motivation should be the bandwidth, not the inference time.Correct. This can be bandwidth or storage. And than FPS to 64 is not a competitor, it's 4 times more bandwidth. But then we already have figure 3 to demonstrate that. We don't need this scenario. Figure 3 is with a fixed PointNet. Table 1 is with re-training. The accuracy with re-training is much better both for us and for FPS. The original purpose I did re-training was to show that we did not over-fit to a specific instance of the classifier, but actually got a representation which separates the classes well. But it's also probably the more common use-case, when you can re-train your network to work on less points. unless you want to only have 1 copy of your task network, and feed it with different number of points in different times (according to network availability, or gpu usage etc). Or if it's a hugae network that you can't afford to re-train.

% Okay, here's the sceario: You have a large ProgressiveNet that is fixed and the question is how best to use it in a client-server scenario. Correct? ProgressiveNet? PointNet Yes. You are correct. This is the scenario that is answerd by figure 3. You want to feed your network with out points, to get better accuracy than FPS....If you can't afford feeding it more points.

% Okay, table2 is not useful without accuracy. We need a graph where the x-axis is FLOPS and y-axis is accuracy and then we can compare different combinations. We will lose. FPS with more points will win.
% Then the x-axis can be the number of samples and y-axis the accuracy. This is figure 3 (for fixed task network) and table 1 (for re-trainable task network). Saveing inference time is a by-product. If it's your main concern - use FPS with more points. If you can't, becaue of bandwith - use \SNET.

% Okay, then we should drop the experiment and give just a single paragraph giving the bottom line that \SNET with PointNet16 is 12 faster at inference time compared to PointNet1024 with a slight degradation in performance. Ok. how does it fit in the scenario - organization of the paper?

% It seems we're dropping the scenarios section and simply add two more experiments the \SNET scalability and the retrieval experiment. Then the reconstruction experiments fits nicely as another "learn to sample" example. And where does table 1 (re-training) fits? I think it's important, to show we make good representations and not just over-fit to a specific instance of the classifier + the numbers are impressive. 

% I would tie it with the description of figure 3. One is used with re-training the other without. Correct? Yes. Then add a paragraph detailing both versions of the experiment and refer to figure 3 and table 1. Ok.

% )} YES. FPS+PointNET will always be faster, but not as accurate.

% Oren, we compare S-NET to FPS for a fixed number of points. Another way to compare is for a fixed number of network parameters. That is, S-NET + PointNet for 16 requires a certain number of parameters. Say this is comparable to FPS with PointNet with 32 points. How do we stack in that case, in terms of accuracy

% PointNet's number of params is not sensitive to the input size. most of the inference time is in the per-point convolutions. But most of the params are in the fully-connected, after the max-pool.

% And how sensitive is the number of params of S-NET to input size? 


% It's senseteive to the OUTPUT size. The last layer is 3*k, so for large k it's the largest layr. S-NET that samples to 16 has 0.2M params, but ProgressiveNet that samples from 1024 to 1024 has 0.95M, the only difference is in the last (output) layer size. the function is Params(k) = 0.16M + 257*3*k. Input size dosen't matter at all for params. not for PointNet and not for S-NET. 0 effect.

% Okay, so S-NET offers a tradeoff between #params and inference time. You increase the number of params but cut inference time. Can you draw a graph/equation for that. Then we can relate it to figure 3/table 1.
% OK. graph or equation?
% FLOPs(k) = 440M*(k/1024) + 35M. 35M is the inference time of S-NET to process 1024 points, it's not sensetive to k. 440M is the inference time of PointNet for 1024 points. The inference time of pointnet is about linear with the number of input points, hence k/1024.

% Okay, we need to add this equation + some explanation to the text. This fits the standard model of using more memory to speed up computation. Notice that here we add less memory when we seep up more.
% K = 512 takes 0.58M extra space, and save 185M FLOPs
% K = 16 takes only 0.18M extra space, and save 398 FLOPs
% Higher sampling ratio = less space + less time. (but still more space than no sampling at all...). And the story is different for ProgressiveNet, as it's space is fixed, but the inference time of PointNet that uses ProgressiveNet points depends on how much points you choose to use. Sent you 2 charts in the email.


%-------------------------------------             ?????????????
% \medskip
% \noindent {\bfseries ?? Multi-task ??} \quad 


==> discussion.tex <==
\section{Discussion}
A natural alternative for our 2-step sampling approach is to multiply each point with a learnable weight, that reflects the point's relevance for the task at hand. This operation is differentiable and can be learned in an end-to-end manner. We tried this approach and it failed, since the distortion of the shape during the training process was too strong. \textbf{\color{red} Oren: Is it worth addressing this? Is there a well-known related problem where this approach is taken? citation need.}

In the reconstruction task framework, \SNET can be viewed as an auto-encoder. But, unlike other auto-encoders, which represent the data in a latent space,  our approach represents the data in \emph{input} space. 
While the reconstruction from both the latent vector and the sampled points differs somewhat from the input, having access to exact samples from the original data has an advantage in many applications, where actual data is essential and approximated data is unacceptable. In addition, the access to some of the original input can be used to further refine the output point cloud. \textbf{\color{red} How?} \textbf{\color{blue} Oren: I think this discussion should be embedded in the reconstruction sub section of the results section. We don't need a separate discussion section}
